Pose Graph Optimization for a MAV Indoor Localization Fusing 5GNR TOA with an IMU

This paper explores the potential of 5G new radio (NR) Time-of-Arrival (TOA) data for indoor drone localization under different scenarios and conditions when fused with inertial measurement unit (IMU) data. Our approach involves performing graph-based optimization to estimate the drone's position and orientation from the multiple sensor measurements. Due to the lack of real-world data, we use Matlab 5G toolbox and QuaDRiGa (quasi-deterministic radio channel generator) channel simulator to generate TOA measurements for the EuRoC MAV indoor dataset that provides IMU readings and ground truths 6DoF poses of a flying drone. Hence, we create twelve sequences combining three predefined indoor scenarios setups of QuaDRiGa with 2 to 5 base station antennas. Therefore, experimental results demonstrate that, for a sufficient number of base stations and a high bandwidth 5G configuration, the pose graph optimization approach achieves accurate drone localization, with an average error of less than 15 cm on the overall trajectory. Furthermore, the adopted graph-based optimization algorithm is fast and can be easily implemented for onboard real-time pose tracking on a micro aerial vehicle (MAV).

==> Sections/0-commented.tex <==
\section{Introduction}

The use of drones for various applications such as inspection, surveillance, and package delivery has rapidly increased in recent years. However, accurate positioning is critical for these applications. While GNSS or GPS is commonly used for positioning, they are ineffective in indoor environments where satellite signals cannot penetrate. Inertial navigation systems (INSs) are another widely used method for indoor localization, but they can accumulate sensor errors over time, resulting in significant position errors if left uncorrected. Therefore, alternative positioning techniques are necessary for indoor drone applications.

The emergence of 5G technology provides new opportunities for indoor drone localization. 5G networks use high-frequency bands that enable the transmission of large amounts of data with low latency, making it possible to perform accurate positioning. In particular, 5G new radio (NR) signals can be used for estimating the drones' positions through multiple measurements of the time of arrival (TOA) radio-frequency (RF) feature. TOA measurements of 5G NR signals can be used to estimate the distance between the drone and base stations (BSs). By fusing TOA measurements with IMU data, accurate 3D positioning of drones can be achieved.

5G technology has emerged as a promising alternative for seamless indoor positioning in recent years. With extended bandwidth ranges and high cell densities, 5G micro BSs can provide accurate time-based measurements, which can be used to compute the ranges to these BSs and enable high-accuracy trilateration-based positioning using time of arrival (TOA), time difference of arrival (TDOA), or round trip time (RTT). This is especially advantageous in indoor environments where GPS signals may not penetrate, and GNSS-based positioning may suffer from poor accuracy and availability.

The increased line-of-sight (LOS) coverage provided by the dense deployment of 5G BSs can also improve the accuracy of range computation, leading to more precise positioning. This makes 5G technology a promising candidate for addressing the limitations of existing indoor positioning systems, which often rely on vision cameras, LiDARs, or radars, and may be affected by environmental factors such as weather conditions.

The emergence of 5G technology has generated significant interest in the research community and the industry due to its potential to enable new and innovative applications. 5G networks use high-frequency bands offering high bandwidth, low latency, and high reliability, making them ideal for high-speed data transfer and low-latency communication applications.

One area where 5G technology has the potential to make a significant impact is indoor localization. As a result, there is a growing demand for indoor localization solutions for various applications, such as industrial automation, asset tracking, and virtual and augmented reality. In these applications, accurate positioning ensures efficient and effective operations.

Due to signal attenuation and multipath effects, traditional localization techniques like GNSS or GPS do not work well in indoor environments. This has led to the development of alternative indoor localization techniques, such as Wi-Fi, Bluetooth, and ultra-Wideband (UWB). However, these techniques have limitations in terms of accuracy and scalability.

Inertial navigation systems (INSs) are widely used for indoor localization without GNSS signals. However, INSs are prone to accumulating sensor errors over time, which can lead to significant position errors if left uncorrected. While this issue can be mitigated by resetting the INS errors with position updates from other sources, such as GNSS, compensating for longer GNSS outages using perception systems has emerged as a promising option. Vision cameras [], LiDARs [], and radars [] have been proposed as alternative positioning sensors, but their performance is heavily dependent on the surrounding environment and weather conditions. Therefore, there is a need for alternative approaches that can provide accurate and robust indoor localization without relying on external sources or environmental factors.

5G technology offers a promising solution for indoor localization due to its ability to provide accurate and reliable positioning information. In particular, 5G NR signals can be used for TOA-based positioning, where the distance between the drone and base stations is estimated based on the time delay of the signals. By fusing TOA measurements with IMU data, accurate 3D positioning of drones can be achieved.


To our knowledge, the use of TOA from 5G NR signals in drone localization has not been extensively investigated, especially in graph-based optimization. Graph-based optimization algorithms are practical for accurate and efficient localization in various applications, and their suitability for 5G-based drone localization has not been fully explored. In this work, we investigate the performance of graph-based optimization algorithms for fusing TOA and IMU data from 5G NR signals in different network configurations and line-of-sight (LOS) scenarios. We demonstrate the potential of 5G-based localization for drone applications and highlight the benefits of combining 5G TOA with simple IMU sensors readily available on most drones.

% (copied)
5G-NR New Radio (5G-NR) is destined to revolutionize the wireless communications as well as user wireless positioning. 5G systems will continue to use the Positioning Reference Signals (PRS) employed now in 4G systems, in order to enable positioning with non-synchronized Base Stations (BS) with an increased performance compared to 4G positioning. PRS are used to measure the delays of the downlink transmissions by correlating the received signal from the base station with a local replica in the receiver. However, the meter- or tens-of-meter-level accuracy provided by these systems has proven not to be enough for some applications, such as safety critical applications, autonomous driving, or aircraft positioning, where cm-level accuracy is needed [5] 5G-NR standard will include dedicated data and pilots (PRS or Positioning Reference Signal) for such a purpose. In addition, 5G-NR will most likely operate at higher frequencies than the current 4G systems, i.e., in the range of mm-Waves. This will allow using higher bandwidths, and, consequently, a higher number of dedicated resources for positioning will be available. G-NR transmissions are more flexible than their predecessor technologies. 5G-NR signals can be transmitted using different numerology FR ranges can be divided into two, namely FR1 for frequencies below 6 GHz and FR2 for frequencies above 24 GHz PRS sequences are pseudo-random sequences with good auto-correlation properties and small cross-correlations to ensure accurate timing measurements. PRS signals are sent in at least one symbol and sub-carrier of a frame during a certain number of consecutive slots. 
%
This research aims to investigate the potential of 5G technology for indoor localization and to evaluate the performance of a system that combines IMU data with time-of-arrival (TOA) measurements from 5G signals. Specifically, we present a real-time approach that utilizes Graph-based Optimization and the GTSAM library to fuse IMU data with TOA measurements from multiple 5G BSs. Our results demonstrate the effectiveness of this approach for indoor localization and show that combining IMU data with 5G TOA measurements can improve the accuracy and robustness of drone positioning in indoor environments.

Background and motivation: Begin by explaining the growing interest in 5G technology and the increasing demand for indoor localization solutions. You could discuss the potential applications of this technology, such as in industrial automation, asset tracking, and virtual and augmented reality.

Research problem: State the research problem you are addressing in your paper. For example, you could say that the accuracy of indoor localization systems is affected by factors such as multipath propagation, signal interference, and environmental conditions and that there is a need to develop more robust and accurate localization solutions.

Objectives and contributions: Outline the objectives of your research and the main contributions of your paper. For example, you could say that your study aims to investigate the use of 5G technology for indoor localization and to evaluate the performance of a system that combines IMU data with time-of-arrival (TOA) measurements. You could also mention that your paper presents a novel approach that uses Graph-based Optimization and the GTSAM library to fuse IMU data with TOA measurements and that your results demonstrate the effectiveness of this approach for indoor localization.

Paper organization: Provide an overview of the structure of your paper. For example, you could say that the paper is organized as follows: Section 2 provides a detailed description of the methodology used in the study, including data collection, signal generation, and data fusion. Section 3 presents the results of the experiments, including an analysis of the performance of the localization system under different scenarios and 5G configurations. Section 4 discusses the implications of the findings and potential directions for future research. Finally, Section 5 summarizes the paper's main contributions and concludes the study.

\section{Related Works}
Regarding localization using 5G, the existing literature can be divided into two main approaches. The first approach focuses on the robotic aspects of localization. These studies often rely on simplistic methodologies such as the extended Kalman filter (EKF) and linear optimization. However, there is a lack of comprehensive sensor fusion frameworks, particularly incorporating inertial measurement unit (IMU) data. On the other hand, another group of studies focuses more on the communication aspects, such as signal analysis and estimation of time of arrival (TOA) and angle of arrival (AOA). These studies often employ simple positioning methods with straightforward scenarios, such as fixed targets. It is important to note that to advance 5G-based localization, there is a need to bridge the gap between the robotic and communication aspects and develop advanced techniques that integrate sensor fusion methodologies to enhance accuracy and reliability.
goes beyond
just localisation by mapping the radio environment simultaneously, taking advantage
of NLOS-rich information about transmitter and receiver positions and environmental
obstacles. This paper proposes joint position and orientation estimation for a mobile target
and the position estimation of reflectors and scatters relying on NLOS paths. Leveraging
AOA, AOD, and TOA for each NLOS path, the receiver’s location is determined only based
on the received signal from one base station in 2D if there are at least three NLOS paths. It is
shown in \citet{chu2021vehicle}, in the NLOS situation, cooperation among vehicles improves situational
awareness and localisation performance, as several cars operate in the same environment
where they might share one or more scatters. This results in a correlated multipath structure
that can contribute to the improved localisation


Their approach primarily emphasizes the analysis of signal characteristics and considers a simplified multilateration scenario for localization. However, it is important to note that their work does not comprehensively address the broader aspects of robotic localization, which encompass more complex scenarios and integration with other sensing modalities.


\citet{Sun2020} combine the angle of arrival (AOA) estimates from 5G base stations and TOA measurements from GNSS satellites to perform hybrid localization mathematical models for GNSS TOA measurements 5G AOA measurements are non-linear. Thus, we employ the Taylor series least square method to linearize the mathematical model and estimate the position solution iteratively. At last, moving averaging is then performed on the raw position estimates to reduce the positioning error further.

\citet{deng2020tdoa}




\citet{zhang2021aoa} generated a fingerprint
dataset of AOA and its corresponding amplitude based on the CSI matrix in a 5G network.
Deep Neural network (DNN) was trained and used as a regressor for online estimation (Indoor localization based on the fifth generation
(5G) wireless communication technology has drawn much attention owing to its potential for supporting location based services.
In this paper, we investigate fingerprint-based localization in
5G indoor environment and propose a 5G indoor intelligent
localization scheme. The proposed scheme takes the advantage
of the large bandwidth and subcarrier spacing of 5G signals
to improve the localization accuracy. First, MUSIC algorithm
is applied for angle of arrival (AoA) estimation based on the
channel state information (CSI) matrix. Both the estimated AoAs
and the corresponding amplitudes are collected as fingerprints.
Second, deep neural network (DNN) is employed for location
estimation. Simulation results show that the proposed scheme
performs well in terms of localization accuracy and stability.
The mean localization accuracy of the proposed scheme is better
than 1.1 m even in the non-line-of-sight environment.)



\citet{pan2021low} Based on the SRS symbol, in an up-link, CFR is estimated for each base station in [110],
and subsequently, TOA and AOA are jointly estimated for localisation. Accuracy below
1 m is acquired. (This paper proposes a novel joint angle-of-arrival (AOA) and path delay (a.k.a. time-of-arrival, TOA) estimation (JADE) method for the fifth generation (5G) signal based positioning system. Conventional methods combine angle and delay into a parameter pair and apply super-resolution methods to the large-dimensional space-time/frequency data matrix. The proposed method reduces the computational overhead on the basis of two observations. Firstly, 5G base stations have unbalanced resolutions in temporal and spatial domains, with temporal resolution much better than spatial resolution, especially for those established for indoor coverage. Therefore, the proposed method employs the iterative adaptive approach (IAA) to resolve multipaths in the TOA domain, then applies the spatial digital beamformer subsequently to obtain AOA estimates. Secondly, based on the Vandermonde structure of the delay signature matrix, fast Fourier transform is employed to accelerate the spectrum computation of the IAA method. Comparing the proposed method with the popular multiple signal classification (MUSIC) based JADE algorithm, the estimation error increases by 72\% and 26\% in numerical simulation and in real-measured channel data, respectively. However, a reduction of nearly three orders for computational cost is achieved.)
)

\citet{111} Localisation under the fingerprinting framework is explored in 
based on CSI, where the transfer learning concept is leveraged to reduce the real-world
training effort. QuaDRiGa is leveraged to obtain synthetic CSI to pre-train the CNN model.


\citet{meng2020study}, angle-based fingerprint localisation is conducted. The fingerprints include the
angles (zenith and azimuth) along with their corresponding power for all observed paths.
To validate the results, simulation is performed by recreating 3D outdoor environments,
including building geometry.  (This paper explores network-side cellular user localization using fingerprints created from the angle measurements enabled by 5G. Our key idea is a binning-based fingerprinting technique that leverages multipath propagation to create fingerprint vectors based on angles of arrival of signals along multiple paths at each user. In network simulations that recreate urban environments with 3D building geometry and base station locations for a major city, our binning-based fingerprinting for 5G achieves significantly lower localization errors with a single base station than signal strength-based fingerprinting for LTE)

AOA-based position estimation in a 5G network was experimentally reported in \cite{menta2019performance}, where EKF was used at edge cloud for localisation. (Cellular systems are undergoing a transformation toward the fifth generation (5G). Envisioned
applications in 5G include intelligent transport system (ITS), autonomous vehicles, and robots as a part of
future roads, factories, and society. These applications rely to a great extent on accurate and timely location
information of connected devices. This paper proposes a pantenna arrayractical scheme for acquiring precise and timely
position information by means of a user–centric ultra–dense network (UDN) architecture based on an edge
cloud. The considered solution consists of estimating and tracking the azimuth angle–of–arrival (AoA) of the
line–of–sight (LoS)–path between a device and multiple transmission–reception points (TRPs), each having
a uniform linear antenna array (ULA). AoA estimates from multiple TRPs are fused into position estimates
at the edge cloud to obtain timely position information. The extensive measurements have been carried
out using a proof–of–concept software–defined–radio (SDR) testbed in order to experimentally assess the
achievable positioning accuracy of the proposed architecture. A realistic UDN deployment scenario has been
considered in which TRPs consist of antenna arrays mounted on lamp posts. Our results show that practical
UDNs can provide sub–meter positioning accuracy of mobile users by employing ULAs with at least four
antennas per TRP and by taking into account the non–idealities of the ULAs’ phase and magnitude response.)


The research of \cite{klus2021neural} is related to receiver localization harnessing AOA under 5G MIMO System and
beam-formed RSS, respectively. (In modern radio networks with large antenna arrays and precise beamforming techniques, accurate user positioning plays a key role in enabling seamless mobility management, link optimization, navigation and safety control. In open and rural areas, Global Navigation Satellite Systems (GNSS) are able to provide high-accuracy and high-reliability positioning performance. However, in urban and densely built-up areas the GNSS performance is typically substantially degraded due to rich scattering and multipath propagation effects. In this paper, we propose a machine learning based solution to boost positioning accuracy in urban areas by (i) obtaining User Equipment (UE) position from beamformed Radio Signal Strength (RSS) measurements and (ii) coherently fusing it with GNSS-based positioning data to enhance overall positioning performance. Based on the obtained numerical results, we were able to achieve a meter-level accuracy with the proposed machine learning model utilizing the beamformed RSS measurements, and subsequently improve the positioning accuracy further via fusion with GNSS data.)

\citet{mendrzik2018joint} goes beyond
just localisation by mapping the radio environment simultaneously, taking advantage
of NLOS-rich information about transmitter and receiver positions and environmental
obstacles. This paper proposes joint position and orientation estimation for a mobile target
and the position estimation of reflectors and scatters relying on NLOS paths. Leveraging
AOA, AOD, and TOA for each NLOS path, the receiver’s location is determined only based
on the received signal from one base station in 2D if there are at least three NLOS paths. It is
shown in \citet{chu2021vehicle}, in the NLOS situation, cooperation among vehicles improves situational
awareness and localization performance, as several cars operate in the same environment
where they might share one or more scatters. This results in a correlated multipath structure
that can contribute to the improved localization

\section{Simulation}



\section{Methodology}
Graph-based optimization is a powerful technique that has gained popularity in recent years due to its ability to estimate the state of a system by minimizing a cost function. This technique is particularly useful when working with non-linear measurement models. It is less sensitive to initialization errors than Bayesian filters like the extended Kalman filter and particle filter. The cost function in graph-based optimization represents the difference between predicted and observed measurements, and the optimization process aims to minimize this difference. 

One of the main advantages of graph-based optimization is its ability to optimize the entire trajectory of a system. This feature is particularly useful in applications where the motion is complex and the measurements are noisy. With traditional filters like the EKF and particle filter, the optimization is performed recursively, and the state estimate is updated sequentially based on each measurement. However, with graph-based optimization, the optimization is performed globally, and the entire trajectory is optimized at once. This means the final state estimate is based on all available measurements, resulting in a more accurate estimate.

\subsection{GTSAM Library and ISAM2}
GTSAM (Georgia Tech Smoothing and Mapping) was used to implement the graph-based optimization approach in this study. GTSAM  is a popular open-source library for implementing graph-based optimization algorithms. It provides a flexible and efficient framework for modeling and solving estimation problems and supports various measurement models and optimization techniques. GTSAM has been successfully used in many applications, including robotics, autonomous driving, and indoor localization.

iSAM2 is an iterative optimization algorithm used in GTSAM for solving complex non-linear problems. It is particularly useful for large-scale problems that would be difficult to solve using traditional optimization techniques. iSAM2 works by incrementally updating the solution as new data becomes available, which makes it more efficient and faster than other methods. It also allows for adding and removing variables and constraints during optimization, making it more flexible than other methods. This makes iSAM2 a powerful tool for optimizing complex systems in real time, which is particularly useful for applications in robotics, autonomous vehicles, and other fields that require real-time optimization of complex systems.

A graph-based optimization is a powerful tool used for fusing different sensor modalities. GTSAM, an open-source C++ library, provides a flexible framework for solving nonlinear least-squares problems. Compared to other methods such as Bayesian filters, GTSAM offers several advantages, including handling complex non-linear systems and incorporating constraints between variables. Furthermore, GTSAM supports various sensor models, making it a versatile tool for fusing different types of sensor data. These advantages make GTSAM an attractive choice for researchers and engineers working on sensor fusion applications.

\section{Experiments}

==> Sections/simulation.tex <==
\section{Simulation of the 5G Communication}
\label{sec:5gsimulation}
% \subsection{Overview of 5G technology}
% In 5G, a dedicated positioning reference signal (PRS) measures delay by correlating the received signal with the known PRS sequence. PRS in 5G is more accurate than LTE (Long-Term Evolution) because it uses higher frequency bands, thus producing a better spatial resolution, employs more advanced signal processing techniques, which reduce interference, and adopts improved time synchronization mechanisms. 5G PRS also offers higher flexibility in its configuration than LTE, enabling greater customization and adaptability to variable network conditions, ultimately contributing to higher accuracy in 5G positioning \cite{Dwivedi2021}.

% \subsection{Simulation Scenarios}


This study uses 5G specifications for indoor base stations to generate PRS signals for the time-of-arrival (TOA) measurements. In our simulation, we used MATLAB 5G Toolbox to generate the resource blocks for 5G NR signals, including the PRS and Physical Downlink Shared Channel (PDSCH) resources. %\blue{The following specifications for PRS are used to generate}. 

Aiming at a realistic simulation of the 5GNR wireless communication, we employ QuaDRiGa (quasi-deterministic radio channel generator) channel simulator~\cite{jaeckel2017quadriga}. For precise channel modeling, it is essential to have information regarding the drone's position, orientation, and velocity. This information is required to accurately account for factors such as the Doppler shift effect. We also assume that both the receiver and all transmitters use omnidirectional antennas. Three scenarios were considered, with different frequencies: QuaDRiGa-Industrial-LOS for 5G Hz, 3GPP-38.901-Indoor-LOS for 28 GHz, and mmMAGIC-Indoor-LOS for 78 GHz.

\begin{itemize}
    \item {\bf QuaDRiGa\_Industrial\_LOS \cite{Jaeckel2019}}: This scenario is designed to replicate a line-of-sight (LOS) environment for industrial applications. The simulation is optimized for frequencies ranging from 2 to 6 GHz and aims to capture the radio propagation behavior typically observed in automation industry halls. The scenario is validated through measurements conducted across five factory halls within Siemens' Nuremberg operational premises.

    \item {\bf 3GPP\_38.901\_Indoor\_LOS \cite{3GPP2018}}: This scenario simulates an indoor environment with LOS frequency conditions the range of  0.5-100 GHz. It aims to encompass various indoor deployment scenarios, such as those commonly found in office buildings and shopping centers. These indoor settings typically consist of open cubicle spaces, private enclosed offices, common areas, corridors, etc.

    \item {\bf mmMAGIC\_Indoor\_LOS \cite{CarneirodeSouza2022}}: This is designed specifically for frequencies in the range of 6-100 GHz and Indoor scenarios with LOS like traditional enclosed offices, semi-closed offices (cubicle areas), and open offices. 

    % The mmMAGIC channel model is a widely used model for wireless communication scenarios. It enables the modeling of MIMO radio channels for specific network configurations. mmMAGIC Indoor LOS is one of the predefined scenarios available in the model, which is used to represent the Line-of-Sight (LOS) environment in indoor wireless communications. It is designed for indoor environments such as offices, commercial buildings, and conference rooms. The scenario incorporates parameters such as the distance between transmitter and receiver, the number of reflecting surfaces, and the penetration loss of the walls, which are used to simulate the wireless channel. This scenario is particularly useful for designing and optimizing wireless communication systems for indoor environments.

\end{itemize}

The simulation configurations for each scenario are provided in~\autoref{tab:configs}.
\begin{table}[h!]
    \centering
    \caption{5G system configurations.}
    \label{tab:configs}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{ M{0.17 \textwidth} M{0.05 \textwidth} M{0.05 \textwidth}  M{0.1 \textwidth}  M{0.05 \textwidth}  M{0.05\textwidth} M{0.04\textwidth} M{0.05\textwidth}   } 
        \Xhline{3\arrayrulewidth}
    \bf Scenario & \bf  Freq (GHz) & \bf Bw (MHz)  & \bf Subcarrier Spacing (KHz) & \bf number of RBs & \bf combsize & \bf SNR  & \bf cyclic prefix\\
    \Xhline{3\arrayrulewidth}
    % \rowcolor{gray!25}
    QuaDRiGa-Industrial-LOS & 5(FR1) & 100  & 30 & 275  & 6 & 10 dB & normal \\
    \Xhline{\arrayrulewidth} 
     3GPP-38.901-Indoor-LOS & 28(FR2)& 200  & 60 & 275  & 6 & 10 dB & normal \\
    \Xhline{1\arrayrulewidth}
    mmMAGIC-Indoor-LOS & 78(FR2)& 400  & 120  & 275 & 6 & 10 dB & normal \\
    \Xhline{3\arrayrulewidth}
    

    \end{tabular}
    }
\end{table}






% \section{simulation Setup}
% Then for chennl simulation three Scenrios for three different 5G frequnecy are considered one FR1 and two in FR2. The scnearios are QuaDRiGa-Industrial-LOS for 5G Hz, 3GPP-38.901-Indoor-LOS for 28 GHz and mmMAGIC-Indoor-LOS for 78 Ghz. PRS (positioing reference singal) pilot siganl is used for finding TOA. the method is that the the received singal at the reciever is correlated with the PRS pattern of that in transmitter and then finding by ananalysing the correaltion profile the delay is calcultaed. IN a usual way, The maximum peak might represent the singal as the LOS path has the highest coeff. However, in reality and even in the simulation, the highest peak is not always the response as the direct path is attenuated by something (NLOS) or there is a constructive interference, making the multipath sum powers. In our simulation to find the asnwer we first put the threshoold for the and fileterd the values below it and then we took the first peak as the response. For now the peak is found by trial and error however in the future it worth to find the mathematically or use AI to find the suitabl peak as the response. IN the figure below we show one example of correlation profile in our simulation where neither the first nor the maximum peak is the response however by using a suitbal threshold we can select the first peak as the response 



% In our simulation, we used MATLAB to generate the resource blocks for 5G NR signals, including the PRS and Physical Downlink Shared Channel (PDSCH) resources.

% The scenario known as QuaDRiGa-Industrial-LOS was developed based on a series of measurements carried out in various production halls with different topologies, under different typical industrial scenarios and conditions. The data obtained from these measurements was processed and used to iteratively calculate the corresponding parameters that can be used in both the 3GPP-NR channel model and the QuaDRiGa model. As a result, a propagation channel model was created that can describe radio propagation behavior in automation industry halls for typical industrial settings. This model is particularly useful for application cases such as automatic guided vehicles and D2D communication in machine production halls. (taken and changed from the paper)
    
    % This scenario simulates a line-of-sight (LOS) environment for industrial applications. The environment consists of large buildings, warehouses, and factories, which create large reflections and diffractions.5 factory halls at operational Siemens premises in Nuremberg . The scenario is designed to simulate frequencies in the range of 2-6 GHz GHz.

% \item {\bf 3GPP\_38.901\_Indoor\_LOS \cite{3gpp2018study}}: This scenario simulates an indoor environment with LOS conditions for frequencies in the range of  0.5-100 GHz. It aims to encompass a wide range of indoor deployment scenarios, such as those commonly found in office buildings and shopping centers. These indoor settings typically consist of open cubicle spaces, private enclosed offices, common areas, corridors, etc.

% The scenario includes typical indoor objects such as walls, furniture, and people, which can cause multipath reflections and diffractions.

% The InH office scenarios are valid for distances up to 150 m and are typically comprised of open cubicle areas, walled offices, open areas, and corridors. (copied from a paper)

% This scenario is intended to capture various typical indoor deployment scenarios, including office
% environments, and shopping malls. The typical office environment is comprised of open cubicle areas, walled
% offices, open areas, corridors etc. The BSs are mounted at a height of 2-3 m either on the ceilings or walls. The
% shopping malls are often 1-5 stories high and may include an open area (or "atrium") shared by several floors.
% The BSs are mounted at a height of approximately 3 m on the walls or ceilings of the corridors and shops (taken from another paper)

% \item {\bf mmMAGIC\_Indoor\_LOS \cite{carneiro2022study}}: This is designed specifically for frequencies in the range of 6-100 GHz and Indoor scenarios with LOS like traditional enclosed offices, semi-closed offices (cubicle areas), and open offices.  


% The chosen propagation scenarios are:
% street canyon, outdoor to indoor, open square (plaza),
% office, shopping mall, airport, stadium and subway (copied from a paper)

% The main objective of the mmMAGIC project (mmMagic, 2017) is to develop advanced channel models for the frequency range of 6–100 GHz. For that purpose, various channel measurements have been conducted for a variety of InH scenarios at multiple frequencies, including 60 GHz. The InH scenarios comprise traditional enclosed offices, semi-closed offices (cubicle areas), and open offices. In this case, the BSs are mounted at a height of 1–5 m and can be placed at the ceilings or on the walls. In addition, channel models were developed for indoor airport scenarios, specifically the gate and the check-in areas, where the BSs should be installed near the ceiling at 4–9 m high. (copied from a paper)

% \end{itemize}

% \subsection{Conclusion}
% Summarize the main points of the 5G section and its relevance to your research.

% The TDE is implemented with a threshold-based estimator, such as in [21], in order to mitigate the effect of multipath. This estimation is based on finding the first peak of the correlation between the received signal and the PRS. The threshold is set to 13 dB (i.e., minimum SNR margin in LTE for neighbour cell detection) below the maximum peak of the correlation function. The PRS periodicity is set to 160 ms, thus 1800 ToA measurements are obtained for 90 positioning occasions. The dynamic scenario is repeated 50 times. The position is estimated using four BSs, i.e., M = 4, with the non-linear least squares (NLS) method, which is implemented with the Gauss-Newton algorithm [24]. A. Assessment of vehicular TDL channel models


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Discussion of 5G's potential for indoor localization}
% Discuss the potential of 5G technology for improving indoor localization in the future, and any challenges that may need to be overcome.

% \subsection{5G Specifications}

% In this study, we used 5G specifications for indoor base stations to generate PRS signals for the time-of-arrival (TOA) measurements. The following 5G specifications were used:

% \begin{itemize}
% \item Frequency band: 3.5 GHz
% \item Bandwidth: 100 MHz
% \item Modulation scheme: 256-QAM
% \item Antenna configuration: 8x8 MIMO
% \item Transmit power: 23 dBm
% \item Antenna height: 2.5 m
% \end{itemize}

% These specifications were used to generate PRS signals for three different scenarios: an empty room, a room with furniture, and a room with obstacles. The specifications were chosen to provide a realistic simulation of indoor 5G communications and to evaluate the performance of the localization system under different 5G configurations.
